Enabling Efficient, Reliable Real-World Reinforcement Learning with Approximate Physics-Based Models

We focus on developing efficient and reliable policy optimization strategies for robot learning with real-world data. In recent years, policy gradient methods have emerged as a promising paradigm for training control policies in simulation. However, these approaches often remain too data inefficient or unreliable to train on real robotic hardware. In this paper we introduce a novel policy gradient-based policy optimization framework which systematically leverages a (possibly highly simplified) first-principles model and enables learning precise control policies with limited amounts of real-world data. Our approach $1)$ uses the derivatives of the model to produce sample-efficient estimates of the policy gradient and $2)$ uses the model to design a low-level tracking controller, which is embedded in the policy class. Theoretical analysis provides insight into how the presence of this feedback controller overcomes key limitations of stand-alone policy gradient methods, while hardware experiments with a small car and quadruped demonstrate that our approach can learn precise control strategies reliably and with only minutes of real-world data.

==> feedback.tex <==
\section{Unravelling the Structure of the Policy Gradient}


This Section introduces our main technical results, which illustrate the benefits of explicitly embedding low-level feedback controllers into the policy class $\set{\pi^\theta}_{\theta \in \Theta}$. With an eye towards long-horizon problems, we demonstrate how low-level controllers which stabilize the closed-loop linearizations along the system trajectories allow for more accurate gradient calculations and yield better-conditioned optimization landscapes. 

As before, we investigate these issues for a single fixed task and then leverage our findings to characterize the multi-task objective \eqref{eq:mult_task}. In particular, note that:
\begin{align}
\small \bar{g}_T(\theta) :=& \mathbb{E}_{\big((x_0^i,\psi^i)_{i=1}^N \sim D^N \big)} \big[\textstyle{\frac{1}{N} \sum_{i=1}^{N}} \widehat{g}_T(\theta;x_0^i, \psi^i)\big] \\ \nonumber
=&\mathbb{E}_{(x_0,\psi) \sim D} \big[\hat{g}_T(\theta;x_0,\psi) \big],
\end{align}
so that the bias of the estimator is given by:
\begin{equation}\label{eq:grad_bias}
    \nabla\mathcal{J}_T(\theta) - \bar{g}_T(\theta) = \mathbb{E}_{(x_0,\psi)\sim \mathcal{D}} \big[\nabla J(\theta;x_0,\psi) - \hat{g}_{T}(\theta;x_0,\psi)\big].
\end{equation}
Moreover, by direct calculation we have:
\begin{equation}
    \nabla^2 \mathcal{J}_T(\theta) = \mathbb{E}_{(x_0,\psi) \sim \mathcal{D}} \big[ \nabla^2 J_T(\theta;x_0,\psi)\big]. 
\end{equation}
Thus, we will be able to directly characterize the expected gradient error $\nabla \mathcal{J}_T(\theta) - \bar{g}_T(\theta)$ and Hessian $\nabla^2 \mathcal{J}_T(\theta)$ by first studying the relevant single-task quantities. 

\subsection{Exponential Blow-up of Gradient Errors}


In this section we will investigate how small errors between the model derivatives and the derivatives of the true dynamics can rapidly explode over time and degrade the quality of the estimate $\hat{g}_T(\theta;x_0,\psi) \approx \nabla  J_T(\theta;x_0)$ as the length of the prediction horizon $T \in \N$ increases. As in Sections \ref{sec:true_grad} and \ref{sec:approx_grad} above, let $(x_0,\psi) \in D \times \Psi$ again denote our fixed task, retaining all previous notation. We focus on how the quality of the approximation:
\begin{equation*}
    \hat{\Phi}_{t,t'}\hat{B}_{t'} \approx \Phi_{t,t'}B_{t'},
\end{equation*}
is affected by point-wise errors in the dynamics:
\begin{equation*}
    \Delta A_{t}^{cl} := 
    \hat{A}_{t}^{cl} - A_{t}^{cl},  \ \ \ \Delta B_{t} := \hat{B}_{t} -B_t,
\end{equation*}
when building up the overall gradient estimate \eqref{eq:approx_grad}. Recall terms of the form $\Phi_{t,t'}B_{t'}$ are the only sources of uncertainty in the gradient of the true cost \eqref{eq:futute_sensitivity}. By defining:
\begin{equation*}
    \Delta \Phi_{t,t'} = \hat{\Phi}_{t,t'}-\Phi_{t,t'},
    \vspace{-0.5em}
\end{equation*}
we can re-write:
\begin{align}\label{eq:blow_up}
  \hat{\Phi}_{t,t'}\hat{B}_{t'} -  \Phi_{t,t'}B_{t'}  &=\Phi_{t,t'}\hat{B}_{t'} + \Delta \Phi_{t,t'} \hat{B}_{t'} - \Phi_{t,t'}B_{t'}\\ \nonumber
   &=\Phi_{t,t'} \Delta B_{t'} + \Delta \Phi_{t,t'} \hat{B}_{t'}\\\nonumber
   & = \Phi_{t,t'} \Delta B_{t'} \\\nonumber
   &+ \textstyle{\big(\sum_{s = t'+1}^{t-1} \Phi_{t,s}\Delta A_{s}^{cl} \hat{\Phi}_{s-1,t'}\big)\hat{B}_{t'}}, \label{eq:blow_up}
\end{align}
where in the last equality we have used the following steps:
\begin{align*}
    \Delta \Phi_{t,t'} &= \hat{\Phi}_{t,t'+1}\hat{A}_{t'+1}^{cl}  -\Phi_{t,t'+1} A_{t'+1}^{cl}\\
    & =    \Phi_{t,t'+1}\hat{A}_{t'+1}^{cl} - \Phi_{t,t'+1}   A_{t'+1}^{cl} +  \Delta \Phi_{t,t'+1} \hat{A}_{t'+1}^{cl}\\
    & = \Phi_{t,t'+1}\Delta A_{t'+1}^{cl} + \Delta \Phi_{t,t'+1}\hat{A}_{t'+1}^{cl},
\end{align*}
which can be applied recursively to yield:
\begin{align*}
   \Delta \Phi_{t,t'} &= \textstyle{\sum_{s = t'}^{t-1} \Phi_{t,s+1}\Delta A_{s}^{cl} \prod_{l =t'+1}^{s} \hat{A}_{l}^{cl} }\\
    &=\textstyle{\sum_{s = t'}^{t-1} \Phi_{t,s+1}\Delta A_{s}^{cl}\hat{\Phi}_{s+1,t'}}.
\end{align*}
The last equality in \eqref{eq:blow_up} provides a clear picture of how inaccuracies in the derivatives of the model are propagated over time. For example, when approximating $\hat{\Phi}_{t,t'}\hat{B}_{t,t'} \approx \Phi_{t,t'}B_{t'}$ the error $\Delta B_{t'}$ is magnified by $\Phi_{t,t'}$, while the error $\Delta A_{t'+1}^{cl}$ is magnified by $\Phi_{t,t'+1}$. The extreme case occurs when the linearizations of the closed-loop dynamics for either the real-world system or the approximate model are unstable. Namely, when there exists $M,\alpha>0$ such that for each $t>t'$ we have either $\|\Phi_{t,t'}\|  > M \alpha^{t-t'}$ or $\|\hat{\Phi}_{t,t'}\|  > M \alpha^{t-t'}$. In this case the extent to which the point-wise errors $\Delta B_{t}$ and $\Delta A_{t}^{cl}$ are magnified grows exponentially with the time horizon $T \in \N$. This demonstrates that in general the quality of the approximation $\hat{g}_T(\theta;x_0,\psi)\approx \nabla\hat{J}(\theta;x_0,\psi)$ will degrade exponentially with the length of the prediction horizon, as many systems we wish to control are open-loop unstable. We use the following simple example to illustrate this point:

\textbf{Running Example:} Consider the scalar case with true and modeled dynamics given respectively by: 
\begin{equation}\label{eq:example}
    x_{t+1} = a x_t + b u_t \ \ \ \text{ and } \ \ \ 
    x_{t+1} = \hat{a}x_t + \hat{b} u_t,
\end{equation}
where $a,\hat{a},b,\hat{b}>0$ and $x_t \in \R$ and $u \in U \subset \R$, where $U$ is a convex set. For simplicity, suppose we only want to obtain a policy for a single fixed task $(x_0,\psi) \in D\times \Psi$, and that we use a policy class of the form $\pi_{t}^\theta(x; x_0,\psi) = \bar{u}_t$ where $\theta = (\bar{u}_t,\dots, \bar{u}_{T-1}) $ and $\bar{u}_t \in U$, and we assume that $U$ is convex. In words, the `policy' in this case is an open-loop sequence of controls $u_t = \bar{u}_t$. In this case, we have $\Phi_{t,t'} = a^{t-t'-1}$ and $\hat{\Phi}_{t,t'}= \hat{a}^{t-t'-1}$. Comparing this with \eqref{eq:blow_up} gives a sense for how the modeling errors $\Delta B_t=(\hat{b}-b)$ and $\Delta A_{t}^{cl} =(\hat{a} -a)$ will be magnified by the unstable dynamics. Note that when we use a `policy' of this form we are effectively using a very basic iterative learning control approach \cite{amann1996iterative,abbeel2006using}.  
 
\begin{comment}
\begin{align}
    \hat{\Phi}_{t,t'}\hat{B}_t-\Phi_{t,t'}B_t &= a^{t-t'-1}(\hat{b}-b) \\ \nonumber
    &+ \sum_{s=t'+1}^{t-1} a^{t-t'-2} (\hat{a}-a) \hat{a}^{s-t'-1}\hat{b}
\end{align}
Note how the errors in the model derivatives $(\hat{b}-b)$ and $(\hat{a} -a)$ are magnified exponentially by the unstable dynamics.
\end{comment}
\subsection{Ill-conditioned Optimization Landscapes}
We next investigate how the Hessian $\nabla^{2} J_T(\theta;x_0,\psi)$ can become ill-conditioned as we increase the time horizon $T\in \N$. Again retaining our previous notation for the fixed instance $(x_0,\psi)\in \R^n \times \Psi$ from above, we demonstrate in \cite{tech_rep} that the Hessian is given by the following formula:
\begin{align}\label{eq:hessian}
 \small  \nabla^2 J_T(\theta;x_0,\psi) &=  \textstyle{\big(\frac{\partial x_T}{\partial \theta}\big)^T \cdot \nabla^2 Q_T(x_T) \cdot \frac{\partial x_T}{\partial \theta} } \\\nonumber
    & + \textstyle{\sum_{t=0}^{T-1} \big(\frac{\partial x_t}{\partial \theta}\big)^T \cdot \frac{\partial^2}{\partial x ^2}H_t(x_t,p_t,\theta) \cdot \frac{\partial x_t}{\partial \theta}}  \\\nonumber
    &+ 2\textstyle{\sum_{t=0}^{T-1}} \big(\frac{\partial x_t}{\partial \theta}\big)^T \cdot \frac{\partial^2}{\partial x \partial \theta}H_t(x_t,p_{t+1},\theta) \\\nonumber
    &+ \textstyle{\sum_{t=0}^{T-1} \frac{\partial^2}{ \partial \theta ^2}H_t(x_t,p_{t+1},\theta)},
\end{align}
where for each $t \in \sp{0,\dots, T}$ we define the closed-loop \emph{Hamiltonian} $H_t \colon \R^n \times \R^{1 \times n} \times \Theta \to \R$ via:
\begin{equation*}
H_t(x,p,\theta) =  \bl p,  F(x,\pi_t^\theta(x)) \br + Q_t^\psi(x) 
+ R_t^\psi(\pi^{\theta}_t(x)),
\end{equation*}
suppressing dependence on $(x_0,\psi)$ for readability. While this expression is more involved than the gradient calculation, we highlight the dependence of this expression on the sensitivities of the state trajectory $\set{\frac{\partial x_t}{\partial \theta}}_{t=1}^{T}$, which were calculated explicitly in \eqref{eq:state_sensitivity}. As we show more formally below, when the linearized dynamics are unstable, and the state trajectories are highly sensitive to changes in the policy, the Hessian will grow exponentially with the horizon. Per the discussion in Section \ref{sec:feedback}, this will make the optimization landscape more difficult to optimize over. We illustrate this point with our example: 

\textbf{Running Example:} Consider again the simple scalar example in equation \eqref{eq:example} with the previously described policy class and fixed task $(x_0,\psi)$. Consider a state tracking cost of the form $Q_t^\psi(x_t) =(x_t-x_t^\psi)Q(x_t-x_t^\psi)$ where $Q>0$ and $\set{x_{t}^\psi}_{t=0}^{T-1}$ represents the desired trajectory. There is no input cost $(R(\cdot) \equiv 0)$ for simplicity. 
 For this example one can calculate: $\frac{\partial^2}{\partial x^2}H_t(x_t,p_{t+1},\theta) =Q$, $
    \frac{\partial^2}{\partial x\partial \theta}H_t(x_t,p_{t+1},\theta) = 0$ and $\frac{\partial^2}{\partial \theta^2}H_t(x_t,p_{t+1},\theta) = 0$ so that $\nabla^2 J_T(\theta;x_0,\psi) = diag\big(\Delta_1, \Delta_2, \dots, \Delta_{T-1} \big)$ where $ \Delta_t =  J(\theta;x_0,\psi) = Q \sum_{s=t+1}^{T} a^{s-t}b$. In this case the loss $J(\theta;x_0,\psi)$ is strongly convex, and the condition number of $\nabla^2 J(\theta;x_0,\psi)$ is $\kappa = \frac{\Delta_{0}}{\Delta_{T-1}}$, which we observe grows exponentially with the time horizon. Per our discussion in Section \ref{sec:background}, when $T$ is large the ill-conditioning of the loss landscape will require small step-sizes to maintain stability of gradient descent schemes, limiting the rate of convergence.  



\subsection{The Benefits of Low-level Feedback Control}

Before formally characterizing the bias of the multi-task gradient estimator $\hat{g}_T^N(\theta)$ and the Hessians $\nabla^2 \mathcal{J}_{T}(\theta)$ we return to our running example to illustrate the benefits of constructing the policy class around a low-level feedback controller: 

\textbf{Running Example:}
Let us again consider the example dynamics in \eqref{eq:example}, the task $(x_0,\psi)$ and the tracking costs $Q_t^\psi,  R_t^\psi$ considered above. However, now suppose that we construct our policy class to be of the form $\pi_t^\theta(x_t;x_0,\psi) =k(\bar{x}_{d,t}-x_t)$ where the policy `parameters' are now  $\theta = (\bar{x}_{d,t}, \dots, \bar{x}_{d,t}) \in \R^{T}$. Namely, in this case the policy parameters specify desired positions at different times which are plugged into a low-level proportional tracking controller which penalizes the `tracking error' $\theta_t-x_t$. In this case the closed loop dynamics are $x_{t+1} = ax_t+bk(\bar{x}_{d,t}-x_t)$ and we have $A_t^{cl} = a-bk$ and $\hat{A}_t^{cl} = \hat{a} - \hat{b} k$. If the gain $k>0$ is chosen such that $|a-bk|<1$ and $|\hat{a} - \hat{b}k|<1$, then the transition matrices $\hat{\Phi}_{t,t'}= (\hat{A}_t^{cl})^{t-t'-1}$ and $\Phi_{t,t'}= (A_t^{cl})^{t-t'-1}$ will both decay exponentially with the difference $t-t'$. Thus, the point-wise errors will not be magnified exponentially for larger time horizons. Moreover, one can show that in this case the Hessian is given by $\nabla^2 J_T(\theta;x_0,\psi) = diag\big(\bar{\Delta}_1, \bar{\Delta}_2, \dots, \bar{\Delta}_{T-1} \big)$, where $\bar{\Delta}_t =  Q \sum_{s=t+1}^{T} (a-bk)^{s-t}b < \frac{1}{1-(a-bk)}Qb$. In this case we see that the loss $J(\theta;x_0,\psi)$ is again strongly convex, but now the condition number of the Hessian $\kappa = \frac{\bar{\Delta}_{0}}{\bar{\Delta}_{T-1}}< \frac{1}{1- (a-bk)}$  is of constant order for all $T \in \N$, indicating that the loss landscape can be more aggressively optimized over by gradient descent methods, per the discussion in Section \ref{sec:background}.  

\begin{remark}
Note that it is not essential for the low-level feedback controller to precisely track the specified desired trajectory. We only require it to prevent the sensitivity of the state trajectory (and the approximate sensitivities we obtain from the simple model) from `blowing up' over longer time horizons. However, because the true dynamics are unknown, we cannot guarantee that $\Phi_{t,t'}$ does not grow exponentially without additional structural assumptions. Nonetheless, in many practical scenarios even coarse low-level controllers can reduce the sensitivity of the state trajectories of the real system. Thus, the primary goal of the theoretical results below is to provide qualitative insight into the benefits of optimizing through a family of `relatively good' feedback controllers, rather than providing specific correctness guarantees. 
\end{remark}
\begin{remark}
It should be noted that certain types of iterative learning control approaches do incorporate feedback mechanisms into the update scheme \cite{jang1995iterative} . However, these approaches primarily use the feedback law to provide a good initialization for the feed-forward control and to prevent the learning process from drifting too far from the desired trajectory during training. Namely, these methods typically do not differentiate through a structured class of feedback controllers as we do in our two examples below, where we use a neural network to tune the tracking controller for a wide range of problems. 
\end{remark}


We are now ready to formalize the preceding intuition, making use of the following technical Assumptions:
\begin{assumption}\label{asm:bounded_traj}
There exists a compact subset $\bar{D}\subset \R^n$ such that for each instance $(x_0,\psi) \in D \times \Psi$ and policy parameter $\theta \in \Theta$ we have $\phi^\theta_{t}(x_0,\psi) \in \bar{D}$ for each $t \in \set{0, 1, \dots ,T}$.
\end{assumption}


\begin{assumption}\label{asm:bounded_derviatives}
The first and second partial derivatives of $Q_t$,\ $R_t$,\ $\pi_{t}^{\theta}$, $F$ and $\hat{F}$ are bounded on the set $\bar{D} \times \Psi \times \Theta$.  
\end{assumption}


 The next assumption bounds the point-wise errors between the derivatives of the model \eqref{eq:approx_dyn}
 and the real world system \eqref{eq:true_dyn}:
\begin{assumption}\label{asm:errors}
Let the set $\bar{D}$ be defined as in Assumption \ref{asm:bounded_traj}. There exist constants $\Delta_A,\Delta_B>0$ such that for each $x \in \bar{D}$, $\psi \in \Psi$ and $\theta \in \theta$ we have for each $t \in \set{0,1,\dots,T-1}$:
\begin{equation*}
  \textstyle  \|\frac{\partial}{\partial x}F(x,\pi_t^\theta(x; x_0,\psi)) -\frac{\partial}{\partial x}\hat{F}(x,\pi_t^\theta(x; x_0,\psi))\| < \Delta_A
\end{equation*}
\begin{equation*}
 \textstyle   \|\frac{\partial}{\partial u}F(x,\pi_t^\theta(x; x_0,\psi)) -\frac{\partial}{\partial u}\hat{F}(x,\pi_t^\theta(x; x_0,\psi))\| < \Delta_{B}
\end{equation*}
\end{assumption}
In the statement of the following assumption, for each $(x_0,\psi,\theta) \in D \times \Psi \times \Theta$ we will let $\Phi_{t,t'}^{(\theta,x_0,\psi)}$ and $\hat{\Phi}_{t,t'}^{(\theta,x_0,\psi)}$ respectively denote the state transition matrices generated by linearizing the true and approximate dynamics functions along the corresponding state trajectory of the real-world system. 
\begin{assumption}\label{asm:transitions}
There exists $M>0$ and $\alpha \in \R$ such that for each $(x_0,\psi,\theta) \in D \times \Psi \times \Theta$ the following holds for $t>t'$:
\begin{equation*}
   \max\set{\|\Phi_{t,t'}^{(\theta,x_0,\psi)}\|,\|\hat{\Phi}_{t,t'}^{(\theta,x_0,\psi)}\|} \leq M \alpha^{t-t'-1}.
\end{equation*}
\end{assumption}

In the following results we will consider the cases where $\alpha>0$, $\alpha =0$ and $\alpha <0$ which correspond, respectively, to cases where the linearizations of the closed-loop dynamics are unstable, marginally stable, and exponentially stable in variation. Our first result characterizes the quality of the gradient estimator \eqref{eq:batch_gradient} on different time horizons:
\begin{theorem}\label{thm:grad_error}
Let Assumptions \ref{asm:bounded_traj}-\ref{asm:transitions} hold. Then there exists $K,W>0$ independent of the parameters $T \in \N$, $M,\Delta_A,\Delta_B$ and $\alpha \in \R$ such that for each $\theta \in \Theta$ we have: \begin{equation*}
\small   \|\nabla \mathcal{J}_T(\theta) -\bar{g}_T(\theta)\| \leq \begin{cases}
  CT^2\alpha^{T}\Delta & \text{ if } \alpha>0 \\
    CT^2 \Delta & \text{ if } \alpha = 0 \\
    CT\Delta & \text{ if } \alpha <0,
    \end{cases} 
\end{equation*}
\begin{equation*}
    \mathbb{E}\bigg[\|\hat{g}_T^N(\theta)-\bar{g}_T(\theta) \|^2 \bigg] \leq \begin{cases}\frac{W T^4\alpha^{2T}}{N} & \text{ if } \alpha>0 \\
    \frac{W T^4}{N}  & \text{ if } \alpha = 0 \\
    \frac{W T^2}{N} & \text{ if } \alpha <0,
    \end{cases}
\end{equation*}
where we have denoted $\Delta = \min\set{\Delta_A,\Delta_B}$ and the expectation in the preceding formula is taken with respect to the randomness in the tasks used to generate $\hat{g}_T^N(\theta)$. 
\end{theorem}
\begin{proof}
We first bound the bias of the gradient:
\begin{align*}
 \|\nabla \mathcal{J}_T(\theta) -\bar{g}_T(\theta)\| &= \|\mathbb{E}[\nabla J_T(\theta;x_0,\psi) - \hat{g}_T(\theta;x_0,\psi)] \| \\
 & \leq \mathbb{E}[\|\nabla J_T(\theta;x_0,\psi) - \hat{g}_T(\theta;x_0,\psi) \|] \\
 &\leq \sup \|\nabla J_T(\theta;x_0,\psi) -\hat{g}_T(\theta;x_0,\psi)\|,
\end{align*}
where the preceding expectations are over $(x_0,\psi)\sim D \times \Psi$ and the supremum is taken over $(x_0,\psi) \in D\times \Psi$. The desired bound on the bias directly follows by applying the bound on the task-specific gradient errors from Lemma \ref{lem:single_grad} in the Appendix. Next, to bound the variance estimate note that:
\begin{align*}
\mathbb{E}[\|\hat{g}_T^N(\theta)-\bar{g}_T(\theta) \|^2] &=\textstyle{\frac{1}{N^2}}\sum_{i=1}^{N}\mathbb{E}[\|\hat{g}_T(\theta;x_0,\psi) -\bar{g}_T(\theta)\|^2] \\
&\leq \textstyle{ \frac{1}{N}  \sup \|\hat{g}_T(\theta;x_0,\psi) -\bar{g}_T(\theta) \|^2 }\\
&\leq\textstyle{ \frac{4}{N} \sup \|\hat{g}_T(\theta;x_0,\psi)\|^2},
\end{align*}
where the first expectation is over $(x_0^i,\psi^i)_{i=1}^{N} \sim \mathcal{D}^N$, the second is with respect $(x_0,\psi)\sim \mathcal{D}$ and the supremums are over $(x_0,\psi) \in D\times \Psi$. The desired bound on the variance follows via a direct application of Lemma \ref{lem:grad_bound} in the Appendix which provides a uniform upper-bound on the gradient estimates. 
\end{proof}



The proofs for Lemmas \ref{lem:grad_bound} and \ref{lem:single_grad} can be found in \cite{tech_rep}. The proof of Lemma \ref{lem:single_grad} uses \eqref{eq:blow_up} to track how the point-wise errors in the dynamics derivatives are propagated, and reflects the fact that low-level feedback can squash these errors over long time horizons when $\alpha <0$, and at least does not magnify them in the marginal case where $\alpha=0$. The proof of Lemma \ref{lem:grad_bound} directly works with the form of the gradient in \eqref{eq:futute_sensitivity}. While the method of bounding the variance in Theorem \ref{thm:grad_error} is quite crude, as a more refined analysis would require additional structural assumptions, it captures intuition that we should expect the gradient estimate to be less noisy in cases where the state trajectories are less sensitive to changes in the policy parameters. In particular, when $\alpha>0$ we may require a very large number of samples at each iteration to avoid unacceptable random fluctuations in the policy parameters. 

Next, we provide a bound on the Hessian: 
\begin{theorem}\label{thm:hessian}
Let Assumptions \ref{asm:bounded_traj},\ref{asm:bounded_derviatives} and \ref{asm:transitions} hold. Then there exists a constant $K>0$ independent of the parameters $T \in \N$, $M$ and $\alpha \in \R$ such that for each $\theta \in \Theta$ we have: \begin{equation*}
   \small \|\nabla^2 \mathcal{J}_T(\theta)\|_2 \leq \begin{cases}
    KT^3\alpha^{T} & \text{ if } \alpha>0 \\
    KT^3 & \text{ if } \alpha = 0 \\
    KT^2 & \text{ if } \alpha <0.
    \end{cases} 
\end{equation*}
\end{theorem}
\begin{proof}
Similar to before we have:
\begin{align*}
    \| \nabla^2 \mathcal{J}_T(\theta)\| &\leq \mathbb{E}_{(x_0,\psi)\sim \mathcal{D}}[\|\nabla^2 J_T(\theta;x_0,\psi)\|] \\
    &\leq \sup_{(x_0,\psi) \in D} \|\nabla^2 J_T(\theta;x_0,\psi) \|.
\end{align*}
The desired bound follows from Lemma \ref{lem:hessian} in the Appendix, which uniformly bounds the task-specific Hessians. 
\end{proof}

The proof of Lemma \ref{lem:hessian} works directly with the form of the Hessian in \eqref{eq:hessian}, and can also be found in \cite{tech_rep}. The bound in Theorem \ref{thm:hessian} captures the notion that optimizing \emph{through} a low-level feedback controller which makes the state trajectories less sensitive to changes in the policy parameters will lead to a better-behaved optimization landscape. Per the discussion in Section \ref{sec:background} this implies that we can more aggressively optimize the objective in this case by using large step-sizes.



\begin{comment}
\subsection{Generalizing to the Multi-instance Objectives}
Next, we apply the bounds from the preceding Section to the more general multi-instance objective in \eqref{eq:mult_task}, bounded the expected error of the gradient estimate $\hat{g}_T^N(\theta)$ as well as the norm of $\nabla^2 J_T(\theta)$. We will then bound the variance of the gradient estimator so that the 

Letting $\hat{g}^N(\theta)\sim \hat{G}_T^N(\theta)$ denote the random variable which produces these estimates, the expected value of the estimator is given by: 
\begin{align}
\bar{G}_T^N(\theta) :=& \mathbb{E}_{\big((x_0^i,\psi^i)_{i=1}^N \sim D^N \big)} \bigg[\frac{1}{N} \sum_{i=1}^{N} \widehat{g}(\theta;x_0^i, \psi^i)\bigg] \\ \nonumber
=&\mathbb{E}_{(x_0,\psi) \sim D} \bigg[\hat{g}_T(\theta;x_0,\psi) \bigg].
\end{align}

We can provide the following bounds on the bias of the gradients estimator and the Hessian of $\mathcal{J}_T(\theta)$: 
\begin{corollary}
Let Assumptions \ref{asm:bounded_traj}-\ref{asm:transitions} hold and let $C,\Delta,\alpha>0$ be as in Theorem \ref{thm:grad_error}. Then for each $\theta \in \Theta$ we have:
\begin{equation}
    \|\nabla\mathcal{J}_T(\theta) - \bar{G}_T^N(\theta)\| \leq\begin{cases}
    CT^2\alpha^{T}\Delta & \text{ if } \alpha>0 \\
    CT^2 \Delta & \text{ if } \alpha = 0 \\
    CT\Delta & \text{ if } \alpha <0.
    \end{cases} 
\end{equation}
\end{corollary}

\begin{corollary}
Let Assumptions \ref{asm:bounded_traj} -\ref{asm:transitions} hold and let $K,\alpha>0$ be as in Theorem \ref{thm:hessian}. Then for each $\theta \in \Theta$ we have:
\begin{equation}
    \|\nabla^2 \mathcal{J}_T(\theta)\| \ \leq \begin{cases}
    KT^3\alpha^{T} & \text{ if } \alpha>0 \\
    KT^3 & \text{ if } \alpha = 0 \\
    KT^2 & \text{ if } \alpha <0.
    \end{cases} 
\end{equation}
\end{corollary}

\begin{lemma}
Let Assumptions \ref{asm:bounded_traj}-\ref{asm:transitions} hold. Then there exists $W>0$ such that for each $\theta \in \Theta$ we have:
\begin{equation*}
    \mathbb{E}\bigg[\|\hat{g}_T^N(\theta) \| \bigg] \leq\begin{cases}\frac{W T^4\alpha^{2T}}{N} & \text{ if } \alpha>0 \\
    \frac{W T^2 \Delta^2}{N}  & \text{ if } \alpha = 0 \\
    \frac{W T^2\Delta^2}{N} & \text{ if } \alpha <0.
    \end{cases}
\end{equation*}
\end{lemma}
\begin{proof}
Using standard properties of the variance of sums of i.i.d. random variables we have:
\begin{align*}
Var(\hat{G}^{N}(\theta)) &= \frac{1}{N}\mathbb{E}_{(x_0,\psi)\sim D}\bigg[ \|\bar{G}(\theta) - \hat{g}(\theta;x_0,\psi) \big\|^2 \bigg]\\
    &\leq \frac{1}{N} \sup_{(x_0,\psi)\in \mathcal{D}} (2\|\hat{g}(\theta;\psi,x_0)\|)^2
\end{align*}
\end{proof}

While this is a very crude bound on the variance of the gradient estimator, it is difficult to refine the estimate much without adding additional structural assumptions to the set-up. Nonetheless, the bound captures the notion that the variance of the gradient estimates will tend to be larger when the linearizations along the closed loop dynamics are unstable, in which case we should expect the state trajectories, and thus also the costs and their gradients, to be more sensitive to changes in the initial condition $x_0 \in D$. 
\end{comment}
